Transversity K Factors for Drell-Yan

The question of the K factor in transversely polarised Drell-Yan (DY) processes is examined. The transverse-spin case is peculiar for the absence of a reference point in deeply inelastic scattering (DIS). Therefore, in order to study more fully the possible effects of higher-order corrections on DY asymmetries, a DIS definition for transversity is devised using a hypothetical scalar (Higgs-like) vertex. The results show that some care may be required in interpreting experimentally extracted partonic transversity, in particular when comparing with model calculations or predictions.

==> texfiles/qq-gp-scattering.tex <==
% mode: -*- TeX:UK:Unix -*-
% e-mail: philip.ratcliffe@uninsubria.it
%——————————————————————————————————————————————————————————————————————————————%
\ProvidesFile{qq-gp-scattering.tex}
  [2004/12/10 v1 DY qq-gphoton scattering diagrams (PGR)]
%——————————————————————————————————————————————————————————————————————————————%
\hspace*{2em}
\parbox[c]{25mm}{%
\begin{fmfgraph*}(25,30)
  \fmftop{i1,o1}
  \fmfbottom{i2,o2}
  \fmf{fermion}{i1,v1}
  \fmf{fermion,label=$p_t$,l.s=right,tension=0.6}{v1,v2}
  \fmf{fermion}{v2,i2}
  \fmf{gluon}{v1,o1}
  \fmf{photon}{v2,o2}
  \fmfv{label=$p_1$,l.a=180}{i1}
  \fmfv{label=$p_2$,l.a=180}{i2}
  \fmfv{label=$k$,l.a=0}{o1}
  \fmfv{label=$q$,l.a=0}{o2}
\end{fmfgraph*}%
}%
\hspace{\stretch{1}}
\parbox[c]{1em}{+}
\hspace{\stretch{1}}
\parbox[c]{25mm}{%
\begin{fmfgraph*}(25,30)
  \fmftop{i1,o1}
  \fmfbottom{i2,o2}
  \fmf{fermion}{i1,v1}
  \fmf{fermion,label=$p_u$,l.s=right,tension=0.6}{v1,v2}
  \fmf{fermion}{v2,i2}
  \fmf{phantom}{v1,o1}
  \fmf{phantom}{v2,o2}
  \fmffreeze
  \fmf{gluon,rubout}{v2,o1}
  \fmf{photon}{v1,o2}
  \fmfv{label=$p_1$,l.a=180}{i1}
  \fmfv{label=$p_2$,l.a=180}{i2}
  \fmfv{label=$k$,l.a=0}{o1}
  \fmfv{label=$q$,l.a=0}{o2}
\end{fmfgraph*}%
}%
\hspace*{2em}
%——————————————————————————————————————————————————————————————————————————————%
%%
%% End of file `qq-gp-scattering.tex'.

